Embodied Image Captioning: Self-supervised Learning Agents for Spatially Coherent Image Descriptions

We present a self-supervised method to improve an agent's abilities in describing arbitrary objects while actively exploring a generic environment. This is a challenging problem, as current models struggle to obtain coherent image captions due to different camera viewpoints and clutter. We propose a three-phase framework to fine-tune existing captioning models that enhances caption accuracy and consistency across views via a consensus mechanism. First, an agent explores the environment, collecting noisy image-caption pairs. Then, a consistent pseudo-caption for each object instance is distilled via consensus using a large language model. Finally, these pseudo-captions are used to fine-tune an off-the-shelf captioning model, with the addition of contrastive learning. We analyse the performance of the combination of captioning models, exploration policies, pseudo-labeling methods, and fine-tuning strategies, on our manually labeled test set. Results show that a policy can be trained to mine samples with higher disagreement compared to classical baselines. Our pseudo-captioning method, in combination with all policies, has a higher semantic similarity compared to other existing methods, and fine-tuning improves caption accuracy and consistency by a significant margin. Code and test set annotations available at https://hsp-iit.github.io/embodied-captioning/

==> tex/fienetuning_semantic_results.tex <==
\begin{table}[t!] 
    \centering
    \scriptsize
    \setlength\tabcolsep{2pt}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{r r r r r c c c c c c}
    \toprule
     & \textbf{Captioner} & \textbf{Pseudo-caption} & \textbf{Policy}  & \textbf{Fine-tuning} & $B_4$ & $M$ & $R_L$ & $CI$ & $SP$ & $CS$ \\
    \midrule
    \multirow{7}{*}{\rotatebox[origin=c]{90}{Gibson Semantic}} & \multirow{7}{*}{CoCa} & - & - & NoFT & 12.15 & 21.47 & 42.83 & 0.63 & 28.30 & 63.30 \\
        & & \multirow{7}{*}{Ours} & \multirow{2}{*}{Random} & Standard & 14.48 & 23.40 & 51.38 & 0.93 & 33.37 & 72.10  \\
    & & & & Triplet & 14.75 & 24.20 & 51.29 & 0.94 & 36.50 & 71.41 \\
    \cmidrule{4-11}
    & &  & \multirow{2}{*}{Frontier} & Standard & 13.11 & 21.56 & 46.67 & 0.80 & 31.33 & 67.63 \\
    & & & & Triplet & 13.48 & 21.82 & 45.82 & 0.76 & 29.38 & 66.28 \\
    \cmidrule{4-11}
    & & & \multirow{2}{*}{CLA} & Standard & 13.29 & 21.37 & 47.87 & 0.74 & 31.39 & 64.92 \\
    & & & & Triplet & 13.56 & 22.01 & 48.23 & 0.81 & 34.14 & 66.09 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparison of captioning performance on Gibson testing sets of model trained using Gibson semantic annotations, varying fine-tuning method and policy. \\ 
    KEYS -- $B_4$: BLEU, $M$: METEOR, $R_L$: ROUGE-L, $CI$: CIDER, $SP$: SPICE, $CS$: cosine similarity between SBERT embedding of prediction and annotation.}
    \label{tab:finetuning_semantic_results}
\end{table}


==> tex/policy_details.tex <==
\begin{table}[tbh]
\centering
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{l}
Map encoder \\
\hline 
$\lbrack$ input $\rbrack$ Two stacked images: $B\times2\times256\times256$   \\     
$\lbrack$ layer 1 $\rbrack$ Max pool 2.\\
$\lbrack$ layer 2 $\rbrack$ Conv. $3^2$, Stride $1^2$, Padding 1, ReLU activ.\\
$\lbrack$ layer 3 $\rbrack$ Max pool 2.\\
$\lbrack$ layer 4 $\rbrack$ Conv. $3^2$, Stride $1^2$, Padding 1, ReLU activ.\\
$\lbrack$ layer 5  $\rbrack$ Max pool 2.\\
$\lbrack$ layer 6  $\rbrack$ Conv. $3^2$, Stride $1^2$, Padding 1, ReLU activ.\\
$\lbrack$ layer 7  $\rbrack$Max pool 2.\\
$\lbrack$ layer 8  $\rbrack$ Conv. $3^2$, Stride $1^2$, Padding 1, ReLU activ.\\
$\lbrack$ layer 9 $\rbrack$ Conv. $3^2$, Stride $1^2$, Padding 1, ReLU activ.\\
\\

Orientation encoder \\
\hline 
$\lbrack$ input $\rbrack$ $B\times 1$   \\     
$\lbrack$ layer 1 $\rbrack$ FC 256.\\
\\

Policy network \\
\hline
$\lbrack$ input $\rbrack$ Map feature $\oplus$ Orient. feature\\
$\lbrack$ layer 1 $\rbrack$ FC 512, ReLU activ.\\
$\lbrack$ layer 2 $\rbrack$ FC 256, ReLU activ.\\
$\lbrack$ layer 3 $\rbrack$ FC 1.\\

\end{tabular}}

\caption{\label{tab:networkparameters}Implementation details for the proposed policy. $B$ is the number of concurrent episodes; $\oplus$ denotes a concatenation operation; Conv denotes 2D convolutional layer; FC denotes fully connected layer.}%; $\odot$ indicates an element-wise product between two tensors.}
\label{tab:}
\end{table}

